MapReduce Meets Fine-Grained Complexity: MapReduce Algorithms for APSP, Matrix Multiplication, 3-SUM, and Beyond

Distributed processing frameworks, such as MapReduce, Hadoop, and Spark are popular systems for processing large amounts of data. The design of efficient algorithms in these frameworks is a challenging problem, as the systems both require parallelism---since datasets are so large that multiple machines are necessary---and limit the degree of parallelism---since the number of machines grows sublinearly in the size of the data. Although MapReduce is over a dozen years old~\cite{dean2008mapreduce}, many fundamental problems, such as Matrix Multiplication, 3-SUM, and All Pairs Shortest Paths, lack efficient MapReduce algorithms. We study these problems in the MapReduce setting. Our main contribution is to exhibit smooth trade-offs between the memory available on each machine, and the total number of machines necessary for each problem. Overall, we take the memory available to each machine as a parameter, and aim to minimize the number of rounds and number of machines. In this paper, we build on the well-known MapReduce theoretical framework initiated by Karloff, Suri, and Vassilvitskii ~\cite{karloff2010model} and give algorithms for many of these problems. The key to efficient algorithms in this setting lies in defining a sublinear number of large (polynomially sized) subproblems, that can then be solved in parallel. We give strategies for MapReduce-friendly partitioning, that result in new algorithms for all of the above problems. Specifically, we give constant round algorithms for the Orthogonal Vector (OV) and 3-SUM problems, and $O(\log n)$-round algorithms for Matrix Multiplication, All Pairs Shortest Paths (APSP), and Fast Fourier Transform (FFT), among others. In all of these we exhibit trade-offs between the number of machines and memory per machine.

==> fastfourier.tex <==
\section{Fast Fourier Transform}\label{sec:fourier}
Fast Fourier transform algorithms compute the discrete Fourier transform of a sequence. The discrete Fourier transform (DFT) is obtained via decomposing a sequence of values into components of different frequencies. Discrete Fourier transform has application to many computational problems such as multiplying two polynomials  in time $O(n \log n)$ where $n$ is the lengths of the input polynomials. We bring a formal definition of the Fourier transform in the following. Given $n$ complex numbers $x_0, x_1, \ldots, x_{n-1}$, the Fourier transformation of $x$ is a sequence $X_0, X_1, \ldots, X_{n-1}$ where we have 
$$X_k = \sum_{j=0}^{n-1} x_j e^{-i2\pi kj/n}$$
for every $0 \leq k < n$. Although it seems from the definition that Fourier transform requires $O(n^2)$ arithmetic operations, the Cooley-Tukey algorithm~\cite{gough1997fft} computes the Fourier transformation in time $O(n \log n)$. The Cooley-Tukey algorithm is based on a divide and conquers approach that divides the input sequence into smaller sequences in each step. In this algorithm, we split the input sequence $x$ into the odd sequence $o$ and even sequence $e$ where $e_j = x_{2j}$ and $o_j = x_{2j+1}$. Next, we recursively compute the Fourier transform of both odd and even sequences and finally merge the solution via an iteration over the computed values in each recursion. Algorithm \ref{alg:fourier} describes the Cooley-Tukey FFT algorithm. In Algorithm \ref{alg:fourier}, we assume w.l.g that the input length ($n$) is a power of 2.

\begin{algorithm}

    \KwData{$n$ complex numbers $x_0, x_1, \ldots, x_{n-1}$}
    \KwResult{A sequence of $n$ complex numbers $X_0, X_1, \ldots, X_{n-1}$}
    \If {$n=1$}{
        \Return($x$)\;
    }\Else{
        $e$ an array of size $n/2$ where $e_j \leftarrow x_{2j}$\;
        $o$ an array of size $n/2$ where $o_j \leftarrow x_{2j+1}$\;
        $X_0, X_1, X_{ n/2  -1} \leftarrow $ \textsf{Cooley-Tukey FFT}($e_0,e_1,\ldots,e_{ n/2  -1}$)\;
        $X_{ n/2 }, X_{ n/2 +1} \ldots, X_{n-1}$ \textsf{Cooley-Tukey FFT}($o_0,o_1,\ldots,o_{ n/2 -1}$)\;
        \For {$k \in [0,n/2-1]$}{
            $X_k \leftarrow X_k + \mathsf{exp}(-2\pi i k/n) X_{k+n/2}$\;
            $X_{k+n/2} \leftarrow X_k - 2\mathsf{exp}(-2\pi i k/n) X_{k+n/2}$\;
        }
        \Return($X$)\;
    }
    
    \caption{\textsf{Cooley-Tukey FFT}($x_0,x_1,\ldots,x_{n-1}$)}     \label{alg:fourier}
\end{algorithm}

As shown in Algorithm \ref{alg:fourier}, it only suffices to compute the Fourier transform of the smaller sequences and based on their results one can compute the Fourier transformation of the input via an iteration. Therefore, this algorithm can be efficiently implemented in the MapReduced model. To this end, we need to have $n^{1-\epsilon}$ computers each with memory $n^{\epsilon}$. In each round of the MapReduce algorithm, we break in the problems into subproblems of smaller size until the whole input for a subproblem fits in the memory of a single machine (i.e., the length of the input for a subproblem is bounded by $n^\epsilon$). When the input sequences are smaller than $n^x$, we compute the DFT of each subproblem via a single machine and in the next MapReduce rounds, we merge the solutions to obtain the DFT of the main problem. This algorithm requiers $O(n^{1-\epsilon})$ machines with memory $O(n^\epsilon)$ and runs in $O(\log n^{1-\epsilon})$ MapReduce rounds.

\begin{theorem}\label{theorem:fft}
The Cooley-Tukey algorithm~\cite{gough1997fft} can be implemented in the MapReduce setting on $O(n^{1-\epsilon})$ computers with memory $O(n^\epsilon)$. This algorithm runs in $O(\log n^{1-\epsilon})$ MapReduce rounds.
\end{theorem}

==> figs/figs.tex <==
\section{Figures}
\mbox{ }

\input{figs/omegas.tex}


\input{figs/omegas2.tex}

\clearpage

\input{figs/epsilons.tex}

\clearpage

\input{figs/machines.tex}

\clearpage


==> figs/figs_2.tex <==
\section{Figures}
\mbox{ }

\input{figs/omegas.tex}


\input{figs/omegas2.tex}

\clearpage

\input{figs/epsilons.tex}

\clearpage

\input{figs/machines.tex}

\clearpage


==> figs/table1.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|c|c|}
\hline
problem & memory & \# of machines & \# MapReduce rounds\\
\hline
\OV\enspace& $\tildorder(n^\epsilon)$ & $O(n^{2(1-\epsilon)})$ & 1\\
(\visible{Theorem \ref{ortho}}) (\visible{\textsf{Work-Efficient}}) &&& \\
\hline
\threesum\enspace& $O(n^\epsilon)$ & $O(n^{2(1-\epsilon)})$ & 2\\
(\visible{Theorem \ref{3sumtheorem}}) (\visible{\textsf{Work-Efficient}})& & & \\
\hline
matrix multiplication& $O(n^\epsilon)$ & $O(n^{\omega^*(2-\epsilon)/2})$ & $O(\log n)$\\
(\visible{Theorem \ref{squarematrixmult}}) (\visible{\textsf{Work-Efficient}})&  &  &\\
\hline
LUP decomposition &  &  & \\
determinant & $\tildorder(n^\epsilon)$ & $\tildorder(n^{\omega^*(2-\epsilon)/2})$ & $O(\log n)$\\
inversion &  &  & \\
\hline
rectangular matrix multiplication& $O(n^\epsilon)$ & $O(n^{\omega^*\langle 1,1,x\rangle(2-\epsilon)/2})$ & $O(\log n)$\\
(\visible{Theorem \ref{imbalancedmatrixmult}}) (\visible{\textsf{Work-Efficient}})& & & \\
\hline
distance multiplication& $O(n^\epsilon)$ & $O(n^{3(1-\epsilon/2)})$ & $O(\epsilon^{-1})$\\
(\visible{Theorem \ref{minplusfirst}})& & & \\
\hline
APSP &  &  & \\
diameter  & & &\\
center & $O(n^\epsilon)$ & $O(n^{3(1-\epsilon/2)})$ & $O(\log n \epsilon^{-1})$\\
negative triangle &  &  & \\
(\visible{Corollary \ref{apsp}})&  &  & \\
\hline
rectangular distance multiplication& $O(n^\epsilon)$ & $O(n^{2(1-\epsilon/2)+(x-\epsilon/2)})$ & $O(\epsilon^{-1})$\\
(\visible{Theorem \ref{imbalancedplusmin}})& & &\\
\hline
APSP for unweighted graphs& $O(n^\epsilon)$ & $O(n^{\machines(\epsilon)})$ & $O(\log ^2 n)$\\
(\visible{Theorem \ref{mainmain}})& & & \\
\hline
%FFT & $O(n^\epsilon)$ & $O(n^{1-\epsilon})$ & $O(\log n^{1-\epsilon})$\\
%(\visible{Theorem \ref{theorem:fft}})& & & \\
%\hline
	\end{tabular}
\caption{The memory, number of machines, and the number of MapReduce rounds of our algorithms. Here $\omega^*$ is the optimal matrix multiplication exponent; for the definition of $\machines(\epsilon)$ see Section \ref{urizwick}. \textsf{Work-Efficient} means that the total running time of the algorithm is asymptotically equal to the best known sequential algorithm for that problem.}\label{table1}
\end{table}

==> figs/table2.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{|c|c|c|}
\hline
problem & $\max\{\textbf{memory}, \textbf{\# of machines}\}$ & \# MapReduce rounds\\
\hline
\OV\enspace & $\tildorder(n^{2/3})$ & 1\\
\hline
\threesum\enspace& $O(n^{2/3})$ & 2\\
\hline
matrix multiplication& $O(n^{2\omega^* / (2 + \omega^*)})$ & $O(\log n)$\\
\hline
LUP decomposition &  &  \\
determinant & $O(n^{2\omega^* / (2 + \omega^*)})$ & $O(\log n)$\\
inversion &  &  \\
\hline
distance multiplication& $O(n^{1.2})$ & 2\\
\hline
APSP &  &   \\
diameter  & & \\
center & $O(n^{1.2})$ & $O(\log n)$\\
negative triangle &  &   \\
\hline
APSP for unweighted graphs& $O(n^{1.145})$ & $O(\log ^2 n)$\\
\hline
FFT & $O(n^{0.5})$ & $O(\log n)$\\
\hline
	\end{tabular}
\caption{The complexity of our MapReduce algorithms when the number of machines is equal to the memory of each machine; $\omega^* \approx 2.3728\ldots$ is the best known exponent for matrix multiplication. }\label{table2}
\end{table}

==> priceof.tex <==
\section{Memory Price of MapReduce}\label{sec:conclusion}
In this paper, we present several MapReduce algorithm whose total
running times are asymptotically equal to the best sequential solutions
known for them. However, the total memory used by all machines
together in these algorithms is more than that of the optimal classic
algorithms. For instance, in \threesum, our algorithm uses
$O(n^{2(1-\epsilon)})$ machines with memory
$O(n^\epsilon)$. Therefore, the total memory of all machines together
is $O(n^{2(1-\epsilon)+\epsilon}) = O(n^{1+(1-\epsilon)})$ and thus,
for $\epsilon < 1$ we use more memory than the optimal sequential
algorithm by a factor of $O(n^{1-\epsilon})$.

This observation raises the question of whether this algorithm can be
improved in terms of total memory? Ideally, we would like the total
memory be equal to that of the optimal sequential algorithm which is
$O(n)$ in case of \threesum. Therefore, in order to design such an
algorithm, we have to use $O(n^{1-\epsilon})$ machines with memory
$O(n^\epsilon)$. However, with $O(n^{1-\epsilon})$ many machines, our
algorithm requires $O(n^{1/2+\epsilon/2})$ memory for each machine
which is greater than what we wish to have by a factor
$O(n^{1/2-\epsilon/2})$. We call this factor the \textit{memory price
  of MapReduce} for our algorithm. 

In the interests of space, we only discuss this concept for \threesum, but
we can apply it to all the problems studied in this paper as well as other 
MapReduce algorithms.
An interesting question is whether
we can reduce the memory price for \threesum or for any other problems, by designing a more sophisticated
algorithm. Of course, any improvement or lower bound on this notion is
of theoretical and practical importance.



==> ssp.tex <==
\section{Second Shortest Path and Replacement Path problem}\label{ssp}
Computing the shortest path between two endpoint $s$ and $t$ is a classic problem with many application in theoretical computer science. Two famous variation of the shortest path problem are the second simple shortest path problem and the replacement path problem. In the replacement path problem we are requested to compute a shortest path between two endpoint $s$ and $t$ that avoids a specific edge $e$. In the second simple shortest path problem we are requested to compute the second simple shortest path between $s$ and $t$. Interestingly as shown in the following problem we can solve both problems efficiently

\begin{theorem}
For $0 \leq \epsilon \leq 2$, the second shortest path and the replacement problem for a specific edge $e$ can be computed with $O(n^{3(1-\epsilon/2)})$ machines with memory $\tildorder(n^{\epsilon})$ in $O(\epsilon^{-1} \log n)$ MapReduce rounds. The total running time of the algorithms for these problems is $\tildorder(\epsilon^{-1} n^3)$.
\end{theorem}

\begin{proof}
A concept that is particularly useful for solving those two problem is the concept of detour. Let $\pi(s,t)=\{s=v_1,v_2,\dots,v_k=t\}$ be the shortest path between $s$ and $t$ in $G$. We say that a simple $u$, $v$ path $D(u,v)$ is a detour of $\pi(s,t)$ if $D(u,v)\cap \pi(s,t) = \{u,v\}$ and $u=v_i$,$v=v_j$ such that $i<j$. A detour $D(u,v)$ si optimal if its length is minimal. Thanks to Lemma 2.1 in~\cite{DBLP:conf/soda/Bernstein10}, we know that for any $e=(v_i,v_{i+1})$ the solution for the replacement path problem for $e$ is of the form $\{s=v_1,v_2,\dots,v_j, D(v_j,v_l), v_l,\dots,v_k=t\}$ for $j\leq i$ and $l\geq i+1$. Furthermore the second simple shortest path is equal to the solution of the replacement path problem for some $e$ in the shortest path $\pi(s,t)$. So, if we could compute all the optimal detours efficiently, we can get a solution for the two problems.

Fortunately in section 2 of~\cite{DBLP:conf/soda/Williams11} it is shown how to reduce the problem of computing all the optimal detours to an APSP problem on an auxiliary graph $G'$. $G'$ is obtained from $G$ by removing all edges in $\pi(s,t)$ from $G$ and by substituting every vertex $v_i$ in the shortest path $\pi(s,t)$ with two vertices $v_i^{in}$ and $v_i^{out}$ so that all the edges going to $v_i$ are added to $v_i^{in}$ and all the edges leaving $v_i$ are added to $v_i^{out}$. It is possible to see that $D(u,v)$ is equal to the shortest path between $u^{out}$ and $v^{in}$.

So to compute the second simple shortest path between $s$ and $t$ in a sequential setting. We can first use the APSP to compute the shortest path between $s$ and $t$. Then we can construct the graph $G'$ and compute the APSP on it to compute all the optimal detours. Finally we can compute the solution of all the Replacement Path problems in $O(n^2)$ and return the best one as a solution for the second simple shortest path between $s$ and $t$. In the next two subsection we show how to implement this strategy in MapReduce using a variation of our APSP algorithm.

\subsection{Second Shortest Path and Replacement Path problem in MapReduce}

In this subsection we show how to implement the described strategy in our parallel model assuming that we have access to a parallel algorithm that is able to return the shortest path between two nodes $s$ and $t$. In the next subsection we show that the shortest path can be computed with $O(n^{3(1-\epsilon/2)})$ machines with memory $\tildorder(n^{\epsilon})$ in $O(\epsilon^{-1} \log n)$ MapReduce rounds with total running time $\tildorder(\epsilon^{-1} n^3)$.

We start by computing the shortest path between $s$ and $t$ using the algorithm mentioned above and the result described in Section~\ref{tikeaval}. Then to compute the graph $G'$, we split the input adjacency matrix in block of size $n^\epsilon$ and we send to each machine a block of the matrix and the list edges in the shortest path between $s$ and $t$ contained in the block. Note that there are at most $n^\epsilon$ such edges. Using this information each machine can modify the block to obtain the same block for the adjacency matrix $G'$. Then we run the APSP algorithm presented in Section~\ref{tikeaval} on $G'$.

Now we have computed the output of APSP for $G$ and $G'$ and the shortest path between $s$ and $t$. Now for every edge $e=(v_i, v_i+1)$ in the shortest path we create $n$ triples containing the length of the shortest path between $s$ and $v_j$, the length of the optimal detour $D(v_j, v_l)$ and the length of the shortest path between $v_l$ and $t$ for all $j\leq i$ and $l\geq i+1$. Note that in total we have $n^3$ triples, so we can sum them up in 1 round of MapReduce using $O(n^{3(1-\epsilon/2)})$ machines with memory $\tildorder(n^{\epsilon})$. Now we are ready to find the second simple shortest path in fact we just need to do this by picking the triple with smaller sum(Note that if we want to solve the Replacement Path problem for an edge $e$ we have to do the same thing after discarding all the path containing $e$) and we can do this in $log n$ rounds.

At this point after $O(log n)$ rounds of MapReduce using $O(n^{3(1-\epsilon/2)})$ machines with memory $\tildorder(n^{\epsilon})$ we know what is the best detour for our problem and so we only need to compute the shortest path between $s$ and $v_j$ in $G$, between $v_j$ and $v_l$ in $G'$ and between $v_l$ and $t$ in $G$ and return them as final solution for our problem.

\subsection{$s$-$t$ shortest path computation via (min,+)-matrix multiplications}

To finish the description of our algorithm we need to describe an algorithm that  return an $s$-$t$ path using $O(n^{3(1-\epsilon/2)})$ machines with memory $\tildorder(n^{\epsilon})$ in $O(\epsilon^{-1} \log n)$ MapReduce rounds with total running time $\tildorder(\epsilon^{-1} n^3)$.

Unfortunately the algorithm cannot construct the path while computing the APSP via (min,+)-matrix multiplications because it would use to much space. To solve this issue instead of keeping all the shortest paths we only keep the length of the shortest paths, the hop-length of the shortest path, a set of $81 \log n$ random vertices selected uniformly at random for every shortest path and an ordering that reflect the vertices position in the shortest path.

First we show that if we have access to the set of points, to the APSP matrix and to the hop length of every shortest path we can solve the problem with high probability. Note that if the shortest path has hop-length $2$ we can just output the two endpoints of the shortest path. If the path is at least of hop-length 3 we have access to a sample of $81\log n $ random vertices selected uniformly at random in the shortest path and their relative order in the shortest path(tie are break arbitrarily). The main idea behind our algorithm is to use the median point in the sample set to split the shortest path in two  shortest path of hop-length bounded by $2/3$ the size of the original shortest path. So by recurse this splitting operation $\log n$ times in parallel we can compute the initial shortest path.

More specifically we start by bounding the probability that the median point in the sample splits the shortest path in two paths of hop-length at most $2/3$ the hop-length of the initial shortest path. Note that if this is not true than more $40.5 \log n$ vertices have to be sampled in the first third or the third third of the shortest path. But the expected number of sample points in any of those sections is bounded by $27\log n$ and all the samples are independent. So by the Chernoff bound we can bound the probability of having more than $36 \log n$ samples in those interval with $O(n^{-3})$. Thus the probability that the median does split one specific shortest path in two shortest path problems with hop-length bounded by $2/3$ the hop-length of the initial shortest path is $1-O(n^{-3})$. 

Now by applying the union bound on all the shortest paths of APSP matrix, we get that all the medians split the shortest paths in in two paths of hop-length smaller than $2/3$ the hop-length of the initial shortest path with probability $1-O(n^{-1})$. So for every shortest path we have access to the two extremes points, its path length and a point that can be used to reduce the problem into 2 subproblems with the size reduced by a constant multiplicative factor. So by recursing $\log n$ times in parallel we can compute the shortest path.

To conclude the proof we need to show that for a specific shortest path it is possible to efficiently sample $81\log n $ random vertices in the shortest path and to keep their ordering. We start by showing that it is possible to obtain the sample and then we explain how to obtain the ordering. The algorithm computes the samples while executing the $(min,+)$-multiplications to compute the APSP. 

In the first step of the APSP algorithm we consider the adjacency matrix and all the computed shortest paths have length one. For those paths we can sample the $81\log n $ random vertices easily because we know the endpoints of every edge. We denote the sampled vertices $s_1,s_2,\dots,s_{81\log n}$, note that this collection is unordered and it can contains the same vertex repeated multiple times. 

After every $(min,+)$-multiplication the algorithm needs to compute a new sample for all the new shortest path discovered by the $(min,+)$-multiplication. Note that all the new paths are obtained by concatenating two already existing shortest paths $P_1$ and $P_2$. So for those two paths the algorithm already has access to their hop-length(it can be easily calculated while computing the $(min,+)$-multiplications), $l_1$ and $l_2$, and their two sampled sets $s'_1,s'_2,\dots,s'_{81\log n}$ and $s''_1,s''_2,\dots,s''_{81\log n}$.  To build the new sample, the algorithm sets for every $i$ $s_i = s'_i$ with probability $l_1/(l_1+l_2)$ and $s_i = s''_i$ with probability $l_2/(l_1+l_2)$. Note that in this way every sample $s_i$ is equal to a specific element in the shortest path with probability $1/(l_1+l_2)$ and so each sample is selected uniformly at random. So the final sample for any specific shortest path is selected uniformly at random(obviously there are dependencies between the samples but this is not an issue because in the proof we consider every shortest path separately.) 

Finally we need to show that the algorithm can keep an ordering of the sampled vertices. For path of length 1 the algorithm can order the sample by knowing the two endpoints. When two paths are concatenated the ordering of the sample is induced by the concatenation of the path and it can be computed efficiently. So an ordering of the sampled vertices can be kept at no additional cost. This concludes the proof.

\end{proof}
